Resilient and Distributed Multi-Robot Visual SLAM: Datasets, Experiments, and Lessons Learned

This paper revisits Kimera-Multi, a distributed multi-robot Simultaneous Localization and Mapping (SLAM) system, towards the goal of deployment in the real world. In particular, this paper has three main contributions. First, we describe improvements to Kimera-Multi to make it resilient to large-scale real-world deployments, with particular emphasis on handling intermittent and unreliable communication. Second, we collect and release challenging multi-robot benchmarking datasets obtained during live experiments conducted on the MIT campus, with accurate reference trajectories and maps for evaluation. The datasets include up to 8 robots traversing long distances (up to 8 km) and feature many challenging elements such as severe visual ambiguities (e.g., in underground tunnels and hallways), mixed indoor and outdoor trajectories with different lighting conditions, and dynamic entities (e.g., pedestrians and cars). Lastly, we evaluate the resilience of Kimera-Multi under different communication scenarios, and provide a quantitative comparison with a centralized baseline system. Based on the results from both live experiments and subsequent analysis, we discuss the strengths and weaknesses of Kimera-Multi, and suggest future directions for both algorithm and system design. We release the source code of Kimera-Multi and all datasets to facilitate further research towards the reliable real-world deployment of multi-robot SLAM systems.

==> sections/additional_results.tex <==


\begin{figure}[!t]
	\centering
	\includegraphics[trim={0 0 0 0},clip, width=1.0\columnwidth]
	{figures/ablations/1207_distributed_alpha-area-plot}
	\caption{{Varying visual similarity threshold ($\alpha$) on \Tunnels dataset}.}\label{fig:ablation_alpha}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[trim={20 20 20 20},clip, width=1.0\columnwidth]{figures/bandwidth_evolution.pdf}
	\caption{Breakdown of message sizes (in log scale) transmitted over time from one robot to another for the four different communication patterns on the \Hybrid dataset.}\label{fig:bandwidth_evolution}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[trim={0 0 0 0},clip, width=1.0\columnwidth]{figures/centralized_system.pdf}
	\caption{Centralized base-line system for comparison against distributed.
		Components are implemented to best resemble their fully-distributed counterparts.}\label{fig:centralized}
\end{figure}

==> sections/mesh_evaluation_table.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{2pt}
\centering
\caption{Mean mesh error (m) across 3 trials.}\label{tab:mesh_evaluation}
\begin{tabular}{c ccc}
\toprule
& \Outdoor & \Tunnels & \Hybrid \\
\midrule
Distributed
& 8.24 $\pm$ 4.49 & 2.57 $\pm$ 0.22 & 2.13 $\pm$ 0.30 \\
Centralized
& 4.47 $\pm$ 0.81 & 2.71 $\pm$ 0.04 & 1.53 $\pm$ 0.02 \\
\midrule
\end{tabular}
\end{table}

==> sections/tab_backend_summary.tex <==
%!TEX root = ../main.tex
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
\caption{\small Summary of Backend Optimization Statistics.}\label{tab:backend_summary}
\begin{tabular}{cl ccccccc}
\toprule
& & \multicolumn{1}{|c|}{Size} & \multicolumn{2}{c|}{Iterations} & \multicolumn{2}{c|}{Optimization Time} & \multicolumn{2}{c}{Metric Error} \\
\midrule
& & \# Poses & \# Max & \# Median & Max(s) & Avg(s) & ATE(m) & AME(m) \\
\midrule
\multirow{3}{*}{Distributed}
& Tunnels & 2832 $\pm$ 6& 1083 $\pm$ 23& 571 $\pm$ 68& 285.55 $\pm$ 31.74& 139.52 $\pm$ 15.52& 4.48 $\pm$ 0.29& 2.62 $\pm$ 0.07\\
& Hybrid & 3201 $\pm$ 6& 1190 $\pm$ 62& 698 $\pm$ 133& 336.98 $\pm$ 26.25& 174.05 $\pm$ 14.97& 7.71 $\pm$ 0.78& 1.9 $\pm$ 0.26\\
& Outdoor & 2383 $\pm$ 1& 735 $\pm$ 327& 344 $\pm$ 31& 196.9 $\pm$ 43.11& 100.92 $\pm$ 11.46& 12.4 $\pm$ 1.92& 4.83 $\pm$ 1.35\\
\midrule
\multirow{3}{*}{Centralized}
& Tunnels & 3053 $\pm$ 4& - & - & 11.51 $\pm$ 1.05& 3.24 $\pm$ 0.28& 4.38 $\pm$ 0.21& 2.58 $\pm$ 0.12\\
& Hybrid & 3508 $\pm$ 1& - & - & 11.44 $\pm$ 0.21& 1.65 $\pm$ 0.16& 5.83 $\pm$ 0.16& 1.58 $\pm$ 0.05\\
& Outdoor & 2647 $\pm$ 0& - & - & 11.49 $\pm$ 2.94& 0.55 $\pm$ 0.12& 9.38 $\pm$ 0.31& 4.99 $\pm$ 0.48\\
\midrule
\end{tabular}
\vspace{-5mm}
\end{table*}

==> sections/tab_datasets.tex <==
%!TEX root = ../main.tex
\begin{table*}[!htbp]
\setlength{\tabcolsep}{2pt}
\centering
\caption{Summary of Multi-Robot Datasets}\label{tab:datasets}
\begin{tabular}{cl ccccccc}
\toprule
& & \# Robots & Traverse(m) & Duration(min) & Vision & Lidar & Dynamic & Environment \\
\midrule
\multirow{4}{*}{NeBula~\cite{Chang22ral-LAMP2}}
& Tunnel & 2 & 2556 & 60 & & \checkmark & & Coal Mine with narrow tunnels \\
& Urban & 3 & 1530 & 60 & & \checkmark & & Multi-level nuclear Power Plant \\
& Finals & 4 & 1224 & 30 & & \checkmark & & Competition Course with urban and mine-like environments\\
& Underground & 4 & 6304 & 60 & & \checkmark & & Limestone Mine with wide expansive caverns\\
\midrule
\multirow{6}{*}{S3E~\cite{Feng22S3E}}
& Square & 3 & 1571 & 8 & \checkmark & \checkmark & \checkmark & Suburban university campus \\
& Library & 3 & 1523 & 8 & \checkmark & \checkmark & \checkmark & Suburban university campus \\
& College & 3 & 2988 & 15 & \checkmark & \checkmark & \checkmark & Suburban university campus \\
& Playground & 3 & 1277 & 5 & \checkmark & \checkmark & \checkmark & Suburban university campus \\
& Dormitory & 3 & 2167 & 11 & \checkmark & \checkmark & \checkmark & Suburban university campus \\
& Indoor & 3 & 1994 & 14 & \checkmark & \checkmark & \checkmark & University campus building \\
\midrule
\multirow{2}{*}{GRACO~\cite{Zhu23Graco}}
& Ground & 6 & 2981 & 9 & \checkmark & \checkmark & \checkmark & Urban university campus \\
& Aerial & 8 & 3938 & 7 & \checkmark & \checkmark & \checkmark & Urban university campus \\
\midrule
% \multirow{4}{*}{M2DGR~\cite{Yin21M2dgr}}
% & Street & 10 & 7728 & 133 & \checkmark & \checkmark & \checkmark &  \\
% & Gate & 3 & 248 & 4 & \checkmark & \checkmark & \checkmark &  \\
% & Hall & 5 & 845 & 14 & \checkmark & \checkmark & \checkmark &  \\
% & Roomdark & 6 & 396 & 7 & \checkmark & \checkmark & \checkmark &  \\
% \midrule
\multirow{3}{*}{*Ours}
& \Outdoor & 6 & 6044 & 19 & \checkmark & \checkmark & \checkmark & Urban university campus \\
& \Tunnels & 8 & 6753 & 28 & \checkmark & \checkmark & \checkmark & Tunnels and hallways \\
& \Hybrid & 8 & 7785 & 27 & \checkmark & \checkmark & \checkmark & Combined urban campus \& indoor tunnels and hallways \\
\midrule
\end{tabular}
\end{table*}

==> sections/tab_frontend_summary.tex <==
%!TEX root = ../main.tex
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\centering
\caption{\small Summary of Front-end Statistics.}\label{tab:frontend_summary}
\begin{tabular}{cl ccc}
\toprule
& & \# Matches & \# Loops & \% Inliers \\
\midrule
\multirow{3}{*}{Distributed}
& Tunnels & 12397 $\pm$ 74& 10620 $\pm$ 70& 20.8 $\pm$ 0.3\\
& Hybrid & 2999 $\pm$ 136& 1252 $\pm$ 30& 26.9 $\pm$ 0.2\\
& Outdoor & 714 $\pm$ 19& 172 $\pm$ 10& 36.5 $\pm$ 2.3\\
\midrule
\multirow{3}{*}{Centralized}
& Tunnels & 12432 $\pm$ 70& 8247 $\pm$ 188& 19.8 $\pm$ 0.4\\
& Hybrid & 3052 $\pm$ 45& 1302 $\pm$ 18& 24.7 $\pm$ 0.5\\
& Outdoor & 732 $\pm$ 6& 182 $\pm$ 5& 37.4 $\pm$ 1.0\\
\midrule
\vspace{-8mm}
\end{tabular}
\end{table}
